Personalized State Anxiety Detection: An Empirical Study with Linguistic Biomarkers and A Machine Learning Pipeline

Individuals high in social anxiety symptoms often exhibit elevated state anxiety in social situations. Research has shown it is possible to detect state anxiety by leveraging digital biomarkers and machine learning techniques. However, most existing work trains models on an entire group of participants, failing to capture individual differences in their psychological and behavioral responses to social contexts. To address this concern, in Study 1, we collected linguistic data from N=35 high socially anxious participants in a variety of social contexts, finding that digital linguistic biomarkers significantly differ between evaluative vs. non-evaluative social contexts and between individuals having different trait psychological symptoms, suggesting the likely importance of personalized approaches to detect state anxiety. In Study 2, we used the same data and results from Study 1 to model a multilayer personalized machine learning pipeline to detect state anxiety that considers contextual and individual differences. This personalized model outperformed the baseline F1-score by 28.0%. Results suggest that state anxiety can be more accurately detected with personalized machine learning approaches, and that linguistic biomarkers hold promise for identifying periods of state anxiety in an unobtrusive way.

==> 2_related_work.tex <==
\section{Background and Related Work} \label{section2-relate-work}


\subsection{Digital Biomarkers and State Anxiety Detection} \label{section2-2}

Digital biomarkers are objective, quantifiable physiological and behavioral markers collected by digital platforms \cite{jacobson2019digital}. Increasingly, ML-based approaches have been used for the purpose of detecting and predicting psychological disorders with digital biomarkers \cite{thieme2020machine}. 
Among studied perspectives (e.g., physiology, behavior), linguistic information is ubiquitous in natural settings, easy to capture, and can be collected in a low-burden and unobtrusive manner, thereby offering a promising tool to detect state anxiety \cite{irvine2020there}. 
 
Several works have found that linguistic biomarkers were able to detect social anxiety. For instance, Salekin \emph{et al.} \cite{salekin2018weakly} proposed a ML technique to detect participants' trait anxiety using audio clips in seconds. Notably, most of work has focused on predicting \emph{trait anxiety} (i.e., general tendency to anxiety) rather than \emph{state anxiety} (i.e., transient reactions) \cite{leal2017trait}. Efforts on state anxiety can offer in-the-moment information to determine when an individual will benefit most from an proper intervention \cite{nahum2018just}, which is the fundamental objective of this present study.

\subsection{Personalized Machine Learning for Mental Health} \label{section2-3}

In ML, personalization consists of tailoring the ML components (e.g., data and model) to achieve personalized outcomes and goals for individuals/cohorts \cite{goldenberg2021personalization}. A growing body of studies have used personalized ML approaches to model psychological data \cite{wang2022personalized}, often with the goal of personalizing the assessment and intervention/recommendation of mental problems \cite{shah2021personalized}. Specifically, some works tailor the data samples that are fed into the model, such as training the model for single individuals \cite{hart2022using}. However, this approach neglects to learn the underlying common patterns within populations and is sometimes overfitted. Also, some researchers have employed ML techniques (e.g., transfer learning, feature selection, domain adaptation) to achieve personalization goals for healthcare \cite{taylor2017personalized,xu2021leveraging}. For example, Taylor \emph{et al.} \cite{taylor2017personalized} built a multitask learning architecture for predicting next-day mood, stress, and health with the design of task-specific layers in the neural networks. Finally, Xu \emph{et al.} \cite{xu2021leveraging} proposed to enable personalized classification and interpretability in the ML pipeline using the collaborative-filtering technique.

==> figures_and_tables/table-related-work.tex <==
\begin{table}[]
\scriptsize
\centering
\renewcommand{\arraystretch}{1.8}
\begin{tabular}{p{1.2cm} p{0.8cm} p{2.7cm} p{2cm} p{1.4cm} p{1.4cm} p{4.2cm}}
\toprule
\textbf{Section} & 
\textbf{Ref.} &
\textbf{Data} &
\textbf{Duration} &
\textbf{Multimodal} &
\textbf{Personalization} & 
\textbf{Outcomes}\\ \hline
\multirow{}{\textbf{Sec. \ref{section2-1}}} 

& \cite{wang2014studentlife,wang2018tracking} & Smartphone data (e.g., accelerometer, GPS, EMAs) & 10 weeks & Yes & No & Understanding and tracking depression \emph{dynamics} with passive sensing data.\\ 

& \cite{tsugawa2015recognizing} & Social media activities (Twitter) & 569.2 days (mean) & No & No & Detecting depression from \emph{twitter} historical activities. \\ 

& \cite{huang2016assessing,boukhechba2017monitoring} & GPS data & 10-14 days & No & No & Assessing college students' social anxiety mainly using \emph{location-based} GPS data. \\ 

& \cite{xu2021leveraging} & Smartphone data (e.g., screen use, GPS, sleep) & 10-16 weeks & Yes & Yes & Detecting depression with \emph{personalized} behavior classification and interpretability. \\ 

& \cite{frommel2021potential,johannes2021assessing} & Game recording & Momentary & No & No & Assessing social anxiety from digital biomarkers in \emph{gaming} behaviors. \\

& \cite{gillespie2017detecting,salekin2018weakly}& Audio recording & Momentary & No & No & Detecting social anxiety and depression from long audio clips. \\

\hline

\multirow{}{\textbf{Sec. \ref{section2-2}}}
& & & \\ 
& & & \\
& & & \\
\hline
\textbf{This work}& & \textbf{Audio and its transcript} &  \textbf{Momentary} & \textbf{Yes} & \textbf{Yes} \\

\bottomrule
\end{tabular}
\caption{Summary of typical studies on ubiquitous assessment and audio/text analysis for mental health and well-being}
\label{table:related-work}
\end{table}


